A hybrid quantum-classical neural network for learning to route

This work studies hybrid quantum-classical neural networks for learning routing heuristics. Specifically, this paper asks whether small quantum neural networks can replace parameter-heavy modules inside a competitive attention-based routing model while maintaining solution quality. For the capacitated vehicle routing problem, encoder feed-forward replacement emerges as the most promising design: it reduces the number of model parameters by 56.6% while keeping the hybrid model close to the classical neural baseline at small and medium instance sizes, although the gap grows for larger instances. This work also compares to classical routing algorithms, which remain highly competitive and often superior on the fixed Euclidean test sets. Our results therefore do not indicate quantum advantage or solver dominance, but identify encoder feed-forward replacement as a viable hybrid-module compression strategy for neural combinatorial optimization.

==> figures/Makefile <==
# generic makefile for latex sources
texfiles := $(wildcard *.tex)
texfiles := $(filter-out Makefile.tex results-table.tex qnn-runs-table.tex qnn-runs-summary-table.tex,$(texfiles))
pdffiles := $(texfiles:.tex=.pdf)
auxdir := "."

.PHONY: all anon clean

all: $(pdffiles)

anon:
	@tmp=$$(mktemp .anon-XXXXXX.tex); \
	printf '%s\n' '\def\anonymous{1}\input{cbctq.tex}' > $$tmp; \
	latexmk -pdf -xelatex -shell-escape -auxdir=$(auxdir) -jobname=cbctq-anon $$tmp; \
	rm -f $$tmp

$(basename $(pdffiles)): %: %.pdf

%.pdf: %.tex
	latexmk -pdf -xelatex -shell-escape -auxdir=$(auxdir) $<

clean:
	latexmk -C

